CodingDINO: Learning to Represent What We See as Code with Agentic Reinforcement Learning

Representations matter. Frontier LLMs increasingly solve complex tasks by writing and executing code, raising the question of how visual inputs can be represented in the same medium. Reconstructing images and videos as executable programs makes appearance, geometry, and temporal dynamics explicit, yielding compositional representations that LLMs can directly inspect, reason over, and edit. Existing vision-to-code methods largely emphasize single-pass generation or inference-time refinement, leaving a gap between using visual feedback and learning from it. We introduce CodingDINO, a unified agentic reinforcement learning (RL) framework for learning internal visual representations through code-based reconstruction. Inspired by DINO, our approach uses observation-to-render consistency as a general learning principle across 2D and 3D images and videos. A unified harness executes and renders SVG, HTML, ThreeJS, Blender, and animation programs, returning visual renders alongside execution diagnostics. Starting from supervised fine-tuning on verified teacher trajectories, multi-turn RL trains the agent to write, render, inspect, and revise code in this harness. Each trajectory is rewarded by execution validity and visual consistency with the target, measured using frozen DINO features and relative depth. Across six image-to-code and video-to-code benchmarks, CodingDINO rivals frontier LLMs such as Opus 5.5 and GPT-6 Astra, ranking first on 10 of 12 headline metrics and in the top three on 10. With no rendering feedback at all, its single-pass variant CodingDINO-Single retains 85.4% of this quality on average. These results position code-based reconstruction as a route to learning reusable internal visual representations, extending DINO's representational ambition to language models that reason and act through code.

==> compile_compat.tex <==
\makeatletter
\@ifpackagelater{microtype}{2025/02/12}{}{%
\def\MT@setup@expansion{%
  \ifnum\pdfoutput<\@ne
    \ifMT@opt@expansion
    \else
      \MT@expansionfalse
    \fi
  \fi
  \ifMT@expansion
    \ifnum\MT@stretch=\m@ne
      \let\MT@stretch\MT@stretch@default
    \fi
    \ifnum\MT@shrink=\m@ne
      \let\MT@shrink\MT@stretch
    \fi
    \ifnum\MT@step=\m@ne
    \MT@requires@pdftex6{%
      \def\MT@step{1 }%
    }{%
      \ifnum\MT@stretch>\MT@shrink
        \ifnum\MT@shrink=\z@
          \@tempcnta=\MT@stretch
        \else
          \@tempcnta=\MT@shrink
        \fi
      \else
        \ifnum\MT@stretch=\z@
          \@tempcnta=\MT@shrink
        \else
          \@tempcnta=\MT@stretch
        \fi
      \fi
      \divide\@tempcnta 5\relax
      \ifnum\@tempcnta=\z@ \@tempcnta=\@ne \fi
      \edef\MT@step{\number\@tempcnta\space}%
    }%
    \fi
    \ifnum\MT@step=\z@
      \MT@warning@nl{The expansion step cannot be set to zero.\MessageBreak
          Setting it to one}%
      \def\MT@step{1 }%
    \fi
    \let\MT@auto\@empty
    \ifMT@auto
      \MT@requires@pdftex4{%
        \ifnum\pdfoutput<\@ne
          \ifMT@opt@auto
            \MT@error{%
              Automatic font expansion only works for PDF output.\MessageBreak
              However, you are creating a DVI file}
             {If you have created expanded fonts instances, remove `auto' from%
              \MessageBreak the package options. Otherwise, you have to switch
              off expansion\MessageBreak completely.}%
          \fi
          \MT@autofalse
        \else
          \def\MT@auto{autoexpand}%
        \fi
      }{%
        \MT@error{%
          The pdftex version you are using is too old for\MessageBreak
          automatic font expansion}%
         {If you have created expanded fonts instances, remove `auto' from\MessageBreak
          the package options. Otherwise, you have to switch off expansion\MessageBreak
          completely, or upgrade pdftex to version 1.20 or newer.}%
        \MT@autofalse
        \def\MT@auto{1000 }%
      }%
    \else
      \MT@requires@pdftex4\relax{%
        \def\MT@auto{1000 }%
      }%
    \fi
    \ifMT@selected
      \let\MT@set@ex@codes\MT@set@ex@codes@s
    \else
      \let\MT@set@ex@codes\MT@set@ex@codes@n
    \fi
    \ifnum\MT@stretch=\z@
      \ifnum\MT@shrink=\z@
        \MT@warning@nl{%
          Both the stretch and shrink limit are set to zero.\MessageBreak
          Disabling font expansion}%
        \MT@expansionfalse
      \fi
    \fi
  \fi
  \ifMT@expansion
    \edef\MT@active@features{\MT@active@features,ex}%
    \MT@adjustspacing\MT@ex@level
    \MT@info@nl{\ifMT@auto A\else Non-a\fi utomatic font expansion enabled
                (level \number\MT@ex@level),\MessageBreak
                stretch: \number\MT@stretch, shrink: \number\MT@shrink,
                step: \number\MT@step, \ifMT@selected\else non-\fi selected}%
    \def\MT@check@step##1{%
      \@tempcnta=\csname MT@##1\endcsname
      \divide\@tempcnta \MT@step
      \multiply\@tempcnta \MT@step
      \ifnum\@tempcnta=\csname MT@##1\endcsname\else
        \MT@warning@nl{The ##1 amount is not a multiple of step.\MessageBreak
                       The effective maximum ##1 is \the\@tempcnta\space
                       (step \number\MT@step)}%
      \fi
    }%
    \MT@check@step{stretch}%
    \MT@check@step{shrink}%
    \MT@check@active@set{ex}%
    \MT@ifdefined@n@TF{showhyphens }{%
      \MT@exp@cs\patchcmd{showhyphens }{\color@begingroup}{\color@begingroup\pdfadjustspacing\z@}
        {\MT@info@nl{Patching command `\string\showhyphens'}}
        {\MT@warning@nl{Unable to patch command `\string\showhyphens'}}%
    }{%
      \CheckCommand*\showhyphens[1]{\setbox0\vbox{\color@begingroup
        \everypar{}\parfillskip\z@skip\hsize\maxdimen\normalfont
        \pretolerance\m@ne\tolerance\m@ne\hbadness\z@\showboxdepth\z@\ ##1\color@endgroup}}
      \gdef\showhyphens##1{\setbox0\vbox{\color@begingroup\pdfadjustspacing\z@
        \everypar{}\parfillskip\z@skip\hsize\maxdimen\normalfont
        \pretolerance\m@ne\tolerance\m@ne\hbadness\z@\showboxdepth\z@\ ##1\color@endgroup}}%
    }%
  \else
    \let\MT@expansion\relax
    \MT@info@nl{No font expansion}%
  \fi
}
}
\makeatother
\DeclareFontShape{T1}{papersans}{b}{it}{<-> s * [0.88] assets/papersans}{}

\pdfglyphtounicode{tfm:cmex10/braceleftBigg}{007B FE04}
\pdfglyphtounicode{tfm:cmex10/bracketleftBigg}{005B FE04}
\pdfglyphtounicode{tfm:cmex10/bracketrightBigg}{005D FE04}
\pdfglyphtounicode{tfm:cmex10/hatwide}{02C6 FE01}
\pdfglyphtounicode{tfm:cmex10/parenleftBig}{0028 FE02}
\pdfglyphtounicode{tfm:cmex10/parenleftBigg}{0028 FE04}
\pdfglyphtounicode{tfm:cmex10/parenrightBig}{0029 FE02}
\pdfglyphtounicode{tfm:cmex10/parenrightBigg}{0029 FE04}
\pdfglyphtounicode{tfm:cmex10/summationdisplay}{2211 FE02}
\pdfglyphtounicode{tfm:cmex10/summationtext}{2211 FE01}

